Champ: Controllable and Consistent Human Image Animation with 3D Parametric Guidance

In this study, we introduce a methodology for human image animation by leveraging a 3D human parametric model within a latent diffusion framework to enhance shape alignment and motion guidance in curernt human generative techniques. The methodology utilizes the SMPL(Skinned Multi-Person Linear) model as the 3D human parametric model to establish a unified representation of body shape and pose. This facilitates the accurate capture of intricate human geometry and motion characteristics from source videos. Specifically, we incorporate rendered depth images, normal maps, and semantic maps obtained from SMPL sequences, alongside skeleton-based motion guidance, to enrich the conditions to the latent diffusion model with comprehensive 3D shape and detailed pose attributes. A multi-layer motion fusion module, integrating self-attention mechanisms, is employed to fuse the shape and motion latent representations in the spatial domain. By representing the 3D human parametric model as the motion guidance, we can perform parametric shape alignment of the human body between the reference image and the source video motion. Experimental evaluations conducted on benchmark datasets demonstrate the methodology's superior ability to generate high-quality human animations that accurately capture both pose and shape variations. Furthermore, our approach also exhibits superior generalization capabilities on the proposed in-the-wild dataset. Project page: https://fudan-generative-vision.github.io/champ.

==> code/simple_video_sample.tex <==
import math
import os
from glob import glob
from pathlib import Path
from typing import Optional

import cv2
import numpy as np
import torch
from einops import rearrange, repeat
from fire import Fire
from omegaconf import OmegaConf
from PIL import Image
from torchvision.transforms import ToTensor

from scripts.util.detection.nsfw_and_watermark_dectection import \
    DeepFloydDataFiltering
from sgm.inference.helpers import embed_watermark
from sgm.util import default, instantiate_from_config


def sample(
    input_path: str = "assets/test_image.png",  # Can either be image file or folder with image files
    num_frames: Optional[int] = None,
    num_steps: Optional[int] = None,
    version: str = "svd",
    fps_id: int = 6,
    motion_bucket_id: int = 127,
    cond_aug: float = 0.02,
    seed: int = 23,
    decoding_t: int = 14,  # Number of frames decoded at a time! This eats most VRAM. Reduce if necessary.
    device: str = "cuda",
    output_folder: Optional[str] = None,
):
    """
    Simple script to generate a single sample conditioned on an image `input_path` or multiple images, one for each
    image file in folder `input_path`. If you run out of VRAM, try decreasing `decoding_t`.
    """
    num_frames_all = num_frames
    if version == "svd":
        num_frames = default(num_frames, 14)
        num_frames = min(num_frames, 14)
        num_steps = default(num_steps, 25)
        output_folder = default(output_folder, "outputs/simple_video_sample/svd/")
        model_config = "scripts/sampling/configs/svd.yaml"
    elif version == "svd_xt":
        num_frames = default(num_frames, 25)
        num_frames = min(num_frames, 25)
        num_steps = default(num_steps, 30)
        output_folder = default(output_folder, "outputs/simple_video_sample/svd_xt/")
        model_config = "scripts/sampling/configs/svd_xt.yaml"
    elif version == "svd_image_decoder":
        num_frames = default(num_frames, 14)
        num_frames = min(num_frames, 14)
        num_steps = default(num_steps, 25)
        output_folder = default(
            output_folder, "outputs/simple_video_sample/svd_image_decoder/"
        )
        model_config = "scripts/sampling/configs/svd_image_decoder.yaml"
    elif version == "svd_xt_image_decoder":
        num_frames = default(num_frames, 25)
        num_frames = min(num_frames, 25)
        num_steps = default(num_steps, 30)
        output_folder = default(
            output_folder, "outputs/simple_video_sample/svd_xt_image_decoder/"
        )
        model_config = "scripts/sampling/configs/svd_xt_image_decoder.yaml"
    else:
        raise ValueError(f"Version {version} does not exist.")

    model, filter = load_model(
        model_config,
        device,
        num_frames,
        num_steps,
    )
    torch.manual_seed(seed)

    path = Path(input_path)
    all_img_paths = []
    if path.is_file():
        if any([input_path.endswith(x) for x in ["jpg", "jpeg", "png"]]):
            all_img_paths = [input_path]
        else:
            raise ValueError("Path is not valid image file.")
    elif path.is_dir():
        all_img_paths = sorted(
            [
                f
                for f in path.iterdir()
                if f.is_file() and f.suffix.lower() in [".jpg", ".jpeg", ".png"]
            ]
        )
        if len(all_img_paths) == 0:
            raise ValueError("Folder does not contain any images.")
    else:
        raise ValueError
    def read_image(input_img_path):
        with Image.open(input_img_path) as image:
            if image.mode == "RGBA":
                image = image.convert("RGB")
            w, h = image.size

            if h % 64 != 0 or w % 64 != 0:
                width, height = map(lambda x: x - x % 64, (w, h))
                image = image.resize((width, height))
                print(
                    f"WARNING: Your image is of size {h}x{w} which is not divisible by 64. We are resizing to {height}x{width}!"
                )

            image = ToTensor()(image)
            image = image * 2.0 - 1.0
        image = image.unsqueeze(0).to(device)
        return image

    for input_img_path in all_img_paths:
        image = read_image(input_img_path)
        H, W = image.shape[2:]
        assert image.shape[1] == 3
        F = 8
        C = 4
        shape = (num_frames, C, H // F, W // F)
        if (H, W) != (576, 1024):
            print(
                "WARNING: The conditioning frame you provided is not 576x1024. This leads to suboptimal performance as model was only trained on 576x1024. Consider increasing `cond_aug`."
            )
        if motion_bucket_id > 255:
            print(
                "WARNING: High motion bucket! This may lead to suboptimal performance."
            )

        if fps_id < 5:
            print("WARNING: Small fps value! This may lead to suboptimal performance.")

        if fps_id > 30:
            print("WARNING: Large fps value! This may lead to suboptimal performance.")

        value_dict = {}
        value_dict["motion_bucket_id"] = motion_bucket_id
        value_dict["fps_id"] = fps_id
        value_dict["cond_aug"] = cond_aug
        value_dict["cond_frames_without_noise"] = image
        value_dict["cond_frames"] = image + cond_aug * torch.randn_like(image)
        value_dict["cond_aug"] = cond_aug
        out_vid_list = list()
        with torch.no_grad():
            with torch.autocast(device):
                for start_index in range(0, num_frames_all, 14):
                    num_frames = min(14, num_frames_all-start_index)
                    shape = (num_frames, C, H // F, W // F)
                    batch, batch_uc = get_batch(
                        get_unique_embedder_keys_from_conditioner(model.conditioner),
                        value_dict,
                        [1, num_frames],
                        T=num_frames,
                        device=device,
                    )
                    c, uc = model.conditioner.get_unconditional_conditioning(
                        batch,
                        batch_uc=batch_uc,
                        force_uc_zero_embeddings=[
                            "cond_frames",
                            "cond_frames_without_noise",
                        ],
                    )

                    for k in ["crossattn", "concat"]:
                        uc[k] = repeat(uc[k], "b ... -> b t ...", t=num_frames)
                        uc[k] = rearrange(uc[k], "b t ... -> (b t) ...", t=num_frames)
                        c[k] = repeat(c[k], "b ... -> b t ...", t=num_frames)
                        c[k] = rearrange(c[k], "b t ... -> (b t) ...", t=num_frames)

                    randn = torch.randn(shape, device=device)
                    #randn = torch.flip(randn_, dims=[0])
                    print(randn[:,0,0,0])
                    # randn[7:14] = randn[0:7]
                    additional_model_inputs = {}
                    additional_model_inputs["image_only_indicator"] = torch.zeros(
                        2, num_frames
                    ).to(device)
                    additional_model_inputs["num_video_frames"] = batch["num_video_frames"]

                    def denoiser(input, sigma, c):
                        return model.denoiser(
                            model.model, input, sigma, c, **additional_model_inputs
                        )

                    samples_z = model.sampler(denoiser, randn, cond=c, uc=uc)
                    model.en_and_decode_n_samples_a_time = decoding_t
                    samples_x = model.decode_first_stage(samples_z)
                    samples = torch.clamp((samples_x + 1.0) / 2.0, min=0.0, max=1.0)


                    samples = embed_watermark(samples)
                    samples = filter(samples)
                    vid = (
                        (rearrange(samples, "t c h w -> t h w c") * 255)
                        .cpu()
                        .numpy()
                        .astype(np.uint8)
                    )
                    last_frame = cv2.cvtColor(vid[-1], cv2.COLOR_RGB2BGR)
                    cv2.imwrite("outputs/last_frame.png", last_frame)
                    image = read_image("outputs/last_frame.png")
                    value_dict["cond_frames_without_noise"] = image
                    value_dict["cond_frames"] = image + cond_aug * torch.randn_like(image)
                    out_vid_list.append(vid)
                os.makedirs(output_folder, exist_ok=True)
                base_count = len(glob(os.path.join(output_folder, "*.mp4")))
                video_path = os.path.join(output_folder, f"{base_count:06d}.mp4")
                print("saving to %s ..."%(video_path))
                writer = cv2.VideoWriter(
                    video_path,
                    # cv2.VideoWriter_fourcc(*"MP4V"),
                    cv2.VideoWriter_fourcc(*'mp4v'),
                    fps_id + 1,
                    (samples.shape[-1], samples.shape[-2]),
                )
                frame_nums = 0
                for vid in out_vid_list:
                    for frame in vid:
                        frame_nums += 1
                        frame = cv2.cvtColor(frame, cv2.COLOR_RGB2BGR)
                        writer.write(frame)
                print("frame_num: %d"%(frame_nums))
                writer.release()


def get_unique_embedder_keys_from_conditioner(conditioner):
    return list(set([x.input_key for x in conditioner.embedders]))


def get_batch(keys, value_dict, N, T, device):
    batch = {}
    batch_uc = {}

    for key in keys:
        if key == "fps_id":
            batch[key] = (
                torch.tensor([value_dict["fps_id"]])
                .to(device)
                .repeat(int(math.prod(N)))
            )
        elif key == "motion_bucket_id":
            batch[key] = (
                torch.tensor([value_dict["motion_bucket_id"]])
                .to(device)
                .repeat(int(math.prod(N)))
            )
        elif key == "cond_aug":
            batch[key] = repeat(
                torch.tensor([value_dict["cond_aug"]]).to(device),
                "1 -> b",
                b=math.prod(N),
            )
        elif key == "cond_frames":
            batch[key] = repeat(value_dict["cond_frames"], "1 ... -> b ...", b=N[0])
        elif key == "cond_frames_without_noise":
            batch[key] = repeat(
                value_dict["cond_frames_without_noise"], "1 ... -> b ...", b=N[0]
            )
        else:
            batch[key] = value_dict[key]

    if T is not None:
        batch["num_video_frames"] = T

    for key in batch.keys():
        if key not in batch_uc and isinstance(batch[key], torch.Tensor):
            batch_uc[key] = torch.clone(batch[key])
    return batch, batch_uc


def load_model(
    config: str,
    device: str,
    num_frames: int,
    num_steps: int,
):
    config = OmegaConf.load(config)
    if device == "cuda":
        config.model.params.conditioner_config.params.emb_models[
            0
        ].params.open_clip_embedding_config.params.init_device = device

    config.model.params.sampler_config.params.num_steps = num_steps
    config.model.params.sampler_config.params.guider_config.params.num_frames = (
        num_frames
    )
    if device == "cuda":
        with torch.device(device):
            model = instantiate_from_config(config.model).to(device).eval()
    else:
        model = instantiate_from_config(config.model).to(device).eval()

    filter = DeepFloydDataFiltering(verbose=False, device=device)
    return model, filter


if __name__ == "__main__":
    Fire(sample)

